Provable Repair of Deep Neural Networks

Deep Neural Networks (DNNs) have grown in popularity over the past decade and are now being used in safety-critical domains such as aircraft collision avoidance. This has motivated a large number of techniques for finding unsafe behavior in DNNs. In contrast, this paper tackles the problem of correcting a DNN once unsafe behavior is found. We introduce the provable repair problem, which is the problem of repairing a network N to construct a new network N' that satisfies a given specification. If the safety specification is over a finite set of points, our Provable Point Repair algorithm can find a provably minimal repair satisfying the specification, regardless of the activation functions used. For safety specifications addressing convex polytopes containing infinitely many points, our Provable Polytope Repair algorithm can find a provably minimal repair satisfying the specification for DNNs using piecewise-linear activation functions. The key insight behind both of these algorithms is the introduction of a Decoupled DNN architecture, which allows us to reduce provable repair to a linear programming problem. Our experimental results demonstrate the efficiency and effectiveness of our Provable Repair algorithms on a variety of challenging tasks.

==> calculus.tex <==
\section{Linear Approximations of Vector Functions}
\label{sec:Calculus}
In this work, we will be using the theory of linear approximations in two major
ways.  First, they will be used to define Decoupled DNNs (\pref{sec:DDNNs})
where we take the activation function for a value channel layer to be a linear
approximation of the activation function for the activation channel. Second,
they will be used to investigate how a DDNN's output varies as the weights of a
particular layer in the value channel are varied. Our key result
(\pref{thm:LinearDDNN}) implies that, when modifying a single layer, the linear
approximation is \emph{exact}, allowing us to encode the repair problem as an
LP.

\onlyfor{arxiv}{\pref{app:Calculus}}{The extended version of this paper} recalls notions of vector calculus. The key definition is
that of the Jacobian:
\begin{definition}
    \label{def:Jacobian}
    Suppose $f : \mathbb{R}^n \to \mathbb{R}^m$ and $\vec{v_0} \in
    \mathbb{R}^n$. We say that $f$ is \emph{differentiable at $\vec{v_0}$} if
    there exists a matrix $J$ such that
    $
        f(\vec{v_0} + \vec{\Delta}) = f(\vec{v_0}) + J\vec{\Delta} + o(\norm{\vec{\Delta}})
    $
    as $\vec{\Delta}$ approaches zero, where $J\vec{\Delta}$ is a matrix-vector
    multiplication. In that case, we say $J$ is the \emph{Jacobian derivative
    (Jacobian) of $f$ at $\vec{v_0}$} and write $D_{\vec{v}} f(\vec{v_0}) = J$.
\end{definition}

In this work we will be using the Jacobian of a DNN with respect to some matrix
parameter. Readers unfamiliar with such concepts are heavily encouraged to
consult~\onlyfor{arxiv}{\pref{app:Calculus}}{the extended version of this paper} for an extended description and examples.

